SHIFT: A Synthetic Driving Dataset for Continuous Multi-Task Domain Adaptation

Adapting to a continuously evolving environment is a safety-critical challenge inevitably faced by all autonomous driving systems. Existing image and video driving datasets, however, fall short of capturing the mutable nature of the real world. In this paper, we introduce the largest multi-task synthetic dataset for autonomous driving, SHIFT. It presents discrete and continuous shifts in cloudiness, rain and fog intensity, time of day, and vehicle and pedestrian density. Featuring a comprehensive sensor suite and annotations for several mainstream perception tasks, SHIFT allows investigating the degradation of a perception system performance at increasing levels of domain shift, fostering the development of continuous adaptation strategies to mitigate this problem and assess model robustness and generality. Our dataset and benchmark toolkit are publicly available at www.vis.xyz/shift.

==> rebuttal_tables/table2.tex <==
\begin{table}[!ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|cccccc}
       \textbf{Frame rate (Hz)}  & 0.25 & 0.5 & 1 & 2 & 5 & 10 \\
       \midrule
       \textbf{\# Frames ($\times$1k)} & 6 & 12 & 25 & 50 & 126 & 252 \\ \midrule
        Seg. (mIoU, \%) & 69.38 & 79.69 & 83.61 & \textbf{83.70} & 83.04 & - \\
        Det. (mAP, \%) & 43.31 & 46.92 & 49.03  & 48.95 & \textbf{49.20} & - \\
        MOT (MOTA, \%) & -  & 58.97 & 60.13 & 63.42 & 65.02 &  \textbf{65.94} \\
    \end{tabular}
    \caption{\footnotesize{Performance of different tasks at increasing sampling rates. Training and testing on the same $505$ sequences from clear-daytime.}}
    \label{tab:frame_rate}
    \vspace{-1em}
\end{table}

==> rebuttal_tables/table3.tex <==
\begin{table*}[!ht]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l|lccl|lccl}
    % \toprule
       \multirow{2}{*}{\textbf{Task}}  & \multicolumn{4}{c|}{\textbf{Rainy}} & \multicolumn{4}{c}{\textbf{Foggy}} \\ 
       & class & $M$ & $\frac{M-M_0}{M_0}$ & wrong predictions (top-2) & class & $M$ & $\frac{M-M_0}{M_0}$ & wrong predictions (top-2) \\
       \midrule
        \multirow{3}{*}{Seg. (mIoU)} & sky & \textbf{27.7} & -69.4\% & building (\textbf{25\%}), bicycle (15\%)  &  wall & 40.1 & -55.7\% & building (17\%), bicycle (8\%) \\
        & traffic sign & 45.1 & -58.4\% & building (13\%), vegetation (10\%) &  vegetation & 40.4 & -54.2\% & sky (19\%), building (17\%) \\
        & person & 46.9 & -52.1\% & car (9\%), building (7\%) & bicycle & 46.7 &  -44.4\% & building (13\%), sky (12\%) \\
        \midrule
        \multirow{3}{*}{Det. (mAP)} & bicycle & 7.5 & -82.1\%  & background (82\%), motor (1\%) &  bicycle & 8.2 & -82.4\% & background (\textbf{89\%}), motor (0.4\%) \\
        & motor & 27.7 & -38.7\% & background (59\%), car (6\%) &  motor & 8.7 & -80.5\% & background (\textbf{86\%}), car (5\%) \\
        & car & 35.9 & -40.6\% & background (58\%), bus (1\%)  & car & 15.6 & -74.2\% & background (\textbf{83\%}), bus (2\%) \\
        % \bottomrule
    \end{tabular}
    \caption{\scriptsize{Top-3 error classes, their performance ($M$) and relative drop w.r.t. the source domain (clear daytime, $M_0$).}}
    \label{tab:error_classes}
\end{table*}


==> sections/0_abstract_v1.tex <==

%%%%%%%%% ABSTRACT
\begin{abstract}
%A robust autonomous driving system needs to cope with wildly varying environmental conditions. 
Adapting to a continuously evolving environment is a safety-critical challenge inevitably faced by all autonomous driving systems.
%
% Existing image- and video-based driving datasets, however, fall short of capturing the continuous domain shifts resulting from realistic environmental changes. 
%
Existing image- and video-based driving datasets, however, fall short of capturing the dynamism of the real world attributable to continuous environmental changes.
% key concept: existing driving datasets are stationary and do not capture continuous distribution shifts   
%
In this paper, we present \thedataset, the largest synthetic dataset for autonomous driving, which comprises continuous shifts in the time of day, cloudiness, rain intensity, fog intensity, and vehicle density. 
%
Featuring a comprehensive sensor suite and annotations for several mainstream perception tasks, \thedataset~allows investigating how perception systems' performance degrades at varying levels of domain shifts and which continuous adaptation strategies best mitigate this problem. 
%
Importantly, using existing datasets we empirically demonstrate that conclusions drawn on our new dataset can translate into the real world. 
% Using \textit{ContinuousSHIFT}, we demonstrate that a sequence-level continuous adaptation can boost performance more significantly than the vanilla discrete adaptation. 
% a range of perception tasks suffer a severe performance loss in out-of-domain conditions and
Dataset and benchmark toolkit will be publicly available. 
\end{abstract}

%We show that a range of perception tasks  suffer a severe performance loss on the 


==> sections/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Recent years have witnessed the remarkable progress of image-based scene understanding approaches in autonomous driving. However, while their accuracy surges on multiple tasks, progress in terms of generalization to various weather~\cite{michaelis2019benchmarking} and lighting~\cite{dai2018dark} conditions has been underwhelming.
% -- their prediction suffers from out-of-distribution (OoD) samples~\cite{blanchard2011generalizing, muandet2013domain}.
% These cause major safety concerns for autonomous vehicles in a widely variable outdoor environment. 
To bridge this gap, recent work focuses on the robustness evaluation that tests model performance under out-of-domain (OoD) conditions, uncertainty estimation~\cite{guo2017calibration, van2020uncertainty, postels2019sampling,gal2016dropout,liu2020simple} that provides accurate confidence levels (\textit{i.e.}, uncertainty calibration), and continuous adaptation methods such as incremental domain adaptation~\cite{IADA2018, lao2020continuous} and test-time adaptation~\cite{wang2020tent,mummadi2021test} that gradually adapts the model to novel domains during training or testing.

A large-scale dataset with continuous domain shifts will unlock multiple research possibilities for the aforementioned areas. Robustness evaluation can discover performance drop with different OoD severities~\cite{michaelis2019benchmarking,hendrycks2021many}. Uncertainty estimation can assess models' calibration under varying levels of difficulty. Continuous domain adaptation, which shows promising results against  artificial corruptions~\cite{wang2020tent, lao2020continuous, wang2020continuously}, can extent its regime to a more practical driving scenario.
However, acquiring a dataset with continuous domain shifts for autonomous driving is particularly challenging.

\input{figures/teaser}

On the one hand, despite numerous real-world driving datasets released to the research community, fine-grained domain labels are absent. For example, BDD100K~\cite{bdd100k} and nuScenes~\cite{caesar2020nuscenes} provide domain labels like ``rainy'' and ``foggy'', but the degrees of raininess and fogginess are not reported since it is hard to quantify from images even for human annotators. We refer to this type of domain shift as \textit{discrete shifts}\footnote{While some datasets have the timestamps, they are not comparable among images since the sunrise/sunset time is varying. Instead, they usually annotate it with discrete labels as ``day'', ``dusk'', ``night'', etc. ~\cite{caesar2020nuscenes, bdd100k}.}. Discrete shifts can be hardly used in continuous learning and the uncertainty calibration under continuous shifts. Additionally, since the length of the sequence is small (\textit{e.g.}, $20\mathrm{sec}$ in nuScenes~\cite{caesar2020nuscenes}, $40\mathrm{sec}$ in BDD100K~\cite{bdd100k}), the environmental changes happening inside each sequence are insufficient. This impedes its usage in evaluating the online test-time adaptation, where a single test sequence needs to cover enough domain shifts, \textit{e.g.}, driving from day to night.
% Difficulties arise when these sequences are used to evaluate the test-time adaptation (TTA) performance, 
Moreover, the degree of domain shifts covered in real-world driving datasets is limited since it is not safe to acquire the data (\textit{e.g.}, heavy fog) and hard to get accurate labels (\textit{e.g.}, dark night) under extreme conditions.
% For example, nuScence has 11.6\% night images.
% This impedes its usage in evaluating the performance of methods in many extreme conditions.

On the other hand, the existing datasets with continuous domain shifts, \textit{e.g.}, CIFAR10/100-C~\cite{michaelis2019benchmarking} and Cityscape-C~\cite{hendrycks2019robustness}, are generated using artificial corruptions, e.g., blurring or additive Gaussian noise, applied to existing datasets. Though carefully designed, such ad-hoc corruptions cannot fully represent the visual shifts in the real world.  
To name a few, in the real world the blurring effect of the fog will be attenuated with the depth growth; the rain will lead to reflective water pounds; the change of time of day will not only affect the brightness but also alter the color of the sky, the saturation of sunlight, the direction of shadows, etc. 
Without realistic physical models, these domain shifts are impossible to produce.
%only with 2D image postprocessing on the existing images.
% where the changes caused by time and weather are more drastic and safety-critical. 

To overcome the limitations of current datasets, we propose ContinuousSHIFT, a new synthetic dataset based on CARLA Simulator~\cite{Dosovitskiy17}. It contains multiple domain shifts corresponding to the safety-critical environmental changes in the real world, including the time of day, cloudiness, rain strength, foggy strength, and vehicle density. The domain shifts are discrete as well as continuous (see Figure~\ref{fig:teaser}). In each sequence of continuous domain shifts, the environment is gradually shifted between two ends along one dimension. To make the shifts comparable, we quantify the degree of shift with a numeric value named \textit{severity}. Frames with the same severity across different sequences have the same environmental parameters. 
%Each frame of the sequence is associated with the value of the degree of change, named \textit{severity}. 
% 

% All the changes are provided in both sequence-level and frame-level. These two aspects of shifts unlock the research possibilities in uncertainty calibration and continuous learning, respectively.




Additionally, the dataset covers diverse environments and supports a comprehensive sensor suite. It has 1,500+ sequences captured from 11 sensors in 8 different scenes. Meanwhile, we provide full annotations for each frame, allowing the usage in 11 perception tasks and the development of multi-task driving systems. The tasks include semantic/instance segmentation, monocular/stereo depth regression, 2D/3D object detection, 2D/3D multiple object tracking (MOT), optical flow estimation, point cloud registration, and forecasting.

% On our new dataset, we conduct extensive evaluations for existing algorithms. 
We benchmark the robustness and uncertainty calibration performance of various perception tasks on our dataset. Moreover, by running similar experiments on real-world datasets, we demonstrate the integrity of conclusions derived from ContinuousSHIFT. We particularly focus on adaptive learning between different domains. We study the effectiveness of continuous adaptation and the impact of domain gap and frame skipping, made possible by the continuous shifts in our dataset.

To summarize, the main contributions of this work are:
\begin{itemize}[leftmargin=1.25em]
\vspace{-0.5em}
\setlength\itemsep{0em}
    \item We construct a novel dataset with discrete and continuous domain shifts of multiple environmental changes crucial to autonomous driving. 
    % ContinuousSHIFT provides comprehensive senors and annotations. 
    To the best of our knowledge, it is the largest synthetic dataset for autonomous driving, \textit{w.r.t.} the number of sequences and the annotation categories. 
    \item We empirically  show that the performance drops between ours and the real-world datasets are comparable on the discrete shifts.
    \item Based on our dataset, we demonstrate new findings of the adaptation performance under different learning strategies for continuously shifted data.
    % We demonstrate that the adaptation on continuously shifted data leads to more significant improvements than domain adaptation with the same amount of data in the target domain, opening new possibilities for the future continuous learning algorithms.
\end{itemize}

==> sections/2_related.tex <==
\section{Related Work}
% The research community have access to a range of autonomous driving datasets, both real-world and synthetic.
%
% Table in Related Work
\begin{table*}[!t]
\centering
\footnotesize
\input{tables/datasets}
\caption{Comparison of annotation and size of image- and video-based driving datasets. \thedataset{} is the largest one among all synthetic datasets and, most importantly, the only one providing realistic continuous domain shifts. ($^\dagger$ BDD100K's MOT set)}
\label{tab:datasets}
\end{table*}
%
\subsection{Driving Datasets}
\paragraph{Real-world datasets} typically focus on a particular subset of perception tasks due to the high cost of data collection and annotation.  
The pioneering real-world dataset KITTI~\cite{geiger2013vision} provides 2D/3D bounding boxes for objects detection and tracking. CamVid~\cite{brostow2009semantic}, Cityscape~\cite{cordts2016cityscapes}, and Mapillary~\cite{neuhold2017mapillary} datasets are designed for instance-level semantic segmentation tasks. HD1K dataset is proposed for optical flow estimation.
% For the point cloud segmentation task, the SemanticKITTI~\cite{} is . 
Recently, many large-scale datasets, \textit{e.g.}, BDD~\cite{bdd100k}, Waymo Open~\cite{sun2020scalability}, and nuScenes~\cite{caesar2020nuscenes}, have been released with multi-task annotations, mainly focusing on object detection and tracking tasks. Our dataset offers a complete set of annotations for all the frames for numerous perception tasks, including those above, enabling multi-task learning in a broader range.

Regarding domain shifts, recent datasets~\cite{pham2020a3d, bdd100k, caesar2020nuscenes, sun2020scalability,mao2021one} provide manually labeled tags for various weather conditions, scene categories, and day periods, but these tags remain coarse-grained. 
%For instance, BDD~\cite{bdd100k} has domain labels of daytime, dusk, night, clear, partly cloudy, overcast, rainy, and foggy. 
In contrast, our dataset provides continuously changing time of day (\textit{i.e.}, Sun's altitude angle) and weather conditions (\textit{i.e.}, cloudiness, rain strength, and fog strength). The fine-grained labels allow future research on robustness and continuous domain adaptation.


\paragraph{Synthetic datasets} are collected using graphic engines and physical simulators. SYNTHIA~\cite{ros2016synthia} contains images and segmentation annotations generated by its simulator. AIODrive~\cite{Weng2020_AIODrive} is produced using CARLA Simulator with multiple sensor support, focusing on high-density long-range LiDAR sets. These datasets have a limited number of sequences and are restricted to discrete domain labels compared to ours; see Table~\ref{tab:datasets}.
Further, video games have also been used for data generation. GTA-V~\cite{richter2016playing} provides the images and segmentation labels captured from a commercial game. However, the low-level control of the environments is hardly accessible in video games, which impedes the collection of continuous shifts.

% The synthetic datasets have domain gaps between the real-world dataset, however 

\paragraph{Adverse Conditions datasets} support the robustness evaluation under different OoD conditions.  Hendrycks \textit{et al.} \cite{hendrycks2019robustness, hendrycks2021many} propose a set of image corruptions applied to ImageNet and CIFAR datasets. Similarly, Michaelis \textit{et al.} \cite{michaelis2019benchmarking} apply corruptions to the existing segmentation dataset, including Pascal, Coco, and Cityscape. 
While these corruptions can be used in a continuous style, they cannot entirely replace realistic domain shifts.


\paragraph{Unsupervised domain adaptation (UDA)} is simultaneously learning on a labeled source domain and an unlabeled target domain, to find robust and transferable features accross domains. UDA is mainly achieved via feature-space alignment~\cite{quinonero2008covariate, sun2017correlation}, domain-consistent regularization~\cite{ganin2015unsupervised, ganin2016domain,hoffman2018cycada} and minimizing a surrogate function of domain gaps~\cite{vu2019advent, saito2019semi}. The discrete shifts in our dataset can be directly used for training and evaluating UDA approaches.

\paragraph{Continual domain adaptation} or incremental domain adaptation ...

\paragraph{Continuous domain adaptation} aims at utilizing a series of intermediate domains between the source and target domain, where domain shifts occur gradually~\cite{lao2020continuous}. Based on the availability of source (labeled) data, it can be further divided into \textit{incremental domain adaptation} (IncDA) and \textit{online test-time adaptation} (OnlineTTA). 
% Incremental Domain Adaptation (IncDA) extends the UDA by introducing , aiming to adapt the model in a non-stationary environment
% % CDA can be further divided into two types, namely \textit{train-time} and \textit{test-time}.
IncDA requires the source data and assumes that the gap between the neighboring domains is small enough such that existing UDA methods can work more efficiently. 
% However, it requires direct access to source and target domains simultaneously, which may not always be feasible.
Meanwhile, OnlineTTA adapts the model to each test sequence separately, sorely based on test samples. It fits any scenarios where access to the training data is not feasible during inference. Recent works~\cite{wang2020tent,mummadi2021test} shows the efficiency of OnlineTTA when applied to the artificial corruptions in ImageNet-C/-R. The continuous shifts in our dataset  facilitate the evaluation of both IncDA and OnlineTTA, and provide a more natural playground for continuous domain adaptation approaches.

% Figure in Dataset
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{images/annotations3.pdf}
    \caption{The annotation set of the RGB camera in our dataset. Each frame is associated with annotations of 2D/3D bounding boxes with tracking identities (visualized by different colors), semantic/instance segmentation, depth map and optical flow label. \label{figure:ann}}
\end{figure*}


==> sections/4_c_multitask.tex <==
\begin{table}[!h]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\input{tables/3dmot_depth}
\caption{Evaluation results for heterogeneous learning of 3D tracking and depth estimation on \thedataset. \bernt{another caption not self-contained and without message for the reader}}
\end{table} \label{tab:multitask_depth}

\subsection{Multitask learning} \label{ssec:exp_multitask}
Multitask learning aims to improve the generalization of a particular task by learning from other tasks~\cite{caruana1997multitask}. 
%
Reducing the number of separate models required for each driving task, multitask learning represents an efficient solution to boost the efficiency of driving algorithms requiring real-time execution with unaffected performance and indirectly promotes robustness by learning more general features~\cite{mao2020multitask}.
%
The wide variety of tasks supported in \thedataset{} provides new opportunities to study how different perception tasks can mutually benefit. 
%
While a body of research~\cite{ruder2017overview,dai2016instance,bdd100k,mao2020multitask} has highlighted the effectiveness of multitask learning, we conduct further experiments on the relationship between 3D MOT and depth estimation.
%
In particular, we rely on the QD3DT~\cite{hu2021monocular} model for 3D MOT and conduct an ablation experiment using the additional dense depth labels to train the depth head.
%
Our results (\autoref{tab:multitask_depth}) show that the tracking performance benefits from the additional dense depth labels, making a stronger case for the collection of dense depth annotations in driving datasets, currently only available in KITTI~\cite{geiger2013vision}.

Full potential is yet to be shown and this dataset allows ...


==> tables/3dmot_depth.tex <==
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccc}
\toprule
\textbf{Training set}      & \textbf{Task} & AP             & MOTA           & MOTP           & IDF$_1$ \\ \midrule
3D MOT & \multirow{2}{*}{3D MOT}  & 0.405          & 0.403          & 0.832          & 0.609         \\
3D MOT + Depth & & \textbf{0.428} & \textbf{0.429} & \textbf{0.847} & \textbf{0.623}  \\
\bottomrule
\end{tabular}

==> tables/exp_semseg.tex <==
\begin{tabular}{llllcccccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Test}} & \multicolumn{5}{c}{\textbf{Weather}}                           & \multicolumn{3}{c}{\textbf{Time of Day}}  \\ \cmidrule(lr){5-9} \cmidrule(lr){10-12} 
                       & & &                       & \textbf{Clear} & P. Cloudy & Overcast & Foggy & Rainy & \textbf{Daytime} & Dawn  & Night \\ \midrule
\textbf{Sem. Seg.} & mIoU (\% $\uparrow$) & Ours                   & Ours                  & 83.61          & 79.32     & 79.43    & 62.39 & 54.58 & 86.11            & 60.75 & 42.79 \\
& & BDD                  & BDD-C                 & 45.56          & 42.56     & 42.36    & \textbf{43.85} & 36.21 & 46.14            & \textbf{40.08} & 19.16 \\
& & BDD + Ours &  BDD-C & \textbf{45.90}          & \textbf{45.38}     & \textbf{45.69}    & 43.06 & \textbf{38.43} & \textbf{46.30}            & 38.85 & \textbf{21.63}

 \\
\midrule
\textbf{2D Detection} & mAP (\% $\uparrow$) & Ours                   & Ours                  & 83.61          & 79.32     & 79.43    & 62.39 & 54.58 & 86.11            & 60.75 & 42.79 \\
& & BDD                  & BDD-C                 & 45.56          & 42.56     & 42.36    & 43.85 & 36.21 & 46.14            & 40.08 & 19.16 \\
& &  BDD + Ours &   BDD-C & -          & -     & -    & - & - & -            & - & - \\
  \midrule
  \textbf{Depth Reg.} & SILog ($\downarrow$) & Ours                   & Ours                  & 31.32 & 33.05 & 33.35 & 46.45 & 52.29 & 35.98 & 43.34 & 73.23 \\
  \midrule
   \textbf{Optical Flow} & RMSE &  Ours &   Ours & -          & -     & -    & - & - & -            & - & - \\
   &  &  HD1K &   HD1K  & -          & -     & -    & - & - & -            & - & - \\
 \bottomrule
\end{tabular}

==> tables/exp_uncertainty.tex <==
\begin{tabular}{llcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} &
  \multirow{2}{*}{\textbf{Method}} &
  \multicolumn{6}{c}{\textbf{Weather}} &
  \multicolumn{4}{c}{\textbf{Time of Day}} &
  \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Overall}}} &
  \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Rank}}} \\ \cmidrule(lr){3-8} \cmidrule(lr){9-12}
 &
   &
  Clear &
  P. Cloudy &
  Overcast &
  Foggy &
  Rainy &
  \multicolumn{1}{l}{\textbf{Avg}} &
  Daytime &
  Dawn &
  Night &
  \multicolumn{1}{l}{\textbf{Avg}} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \midrule
\multirow{5}{*}{{BDD100K}} & Softmax   & 86.39 & 85.40 & 79.08 & 82.80 & 86.37 & 77.99 & 76.57 & 85.57 & 85.56 & 81.09 & 83.32 & 2 \\
                      & MCDropout & 50.07 & 50.06 & 50.09 & 50.08 & 50.06 & 49.95 & 50.05 & 50.13 & 49.98 & 50.03 & 50.00 & 5 \\
                       & Ensemble  & 80.50 & 77.49 & 77.05 & 81.45 & 80.50 & 78.16 & 86.68 & 87.97 & 87.19 & 82.36 & 84.77 & 1 \\
                       & SNGP      & 52.03 & 50.29 & 51.99 & 51.59 & 52.04 & 52.68 & 52.19 & 55.35 & 57.43 & 53.84 & 55.63 & 4 \\
                       & MIR       & 75.11 & 81.53 & 55.57 & 72.45 & 75.12 & 68.39 & 69.33 & 72.71 & 61.53 & 69.20 & 65.36 & 3 \\
                       \midrule
\multirow{5}{*}{{Ours}}  & Softmax   & 95.18 & 72.17 & 55.87 & 81.59 & 95.18 & 84.11 & 85.63 & 73.13 & 47.36 & 84.89 & 66.12 & 2 \\
                        & MCDropout & 50.38 & 49.94 & 49.96 & 50.14 & 50.31 & 50.10 & 50.14 & 50.15 & 50.09 & 50.16 & 50.12 & 5 \\
                       & Ensemble  & 68.73 & 60.56 & 52.57 & 67.98 & 68.74 & 48.44 & 77.67 & 61.42 & 67.84 & 71.26 & 69.55 & 1 \\
                       & SNGP      & 79.58 & 70.52 & 53.18 & 68.81 & 79.50 & 74.63 & 79.43 & 63.48 & 45.76 & 69.87 & 57.81 & 4 \\
                       & MIR       & 79.10 & 61.67 & 44.14 & 73.54 & 79.10 & 59.08 & 80.92 & 59.31 & 52.42 & 71.90 & 62.16 & 3 \\
                       \bottomrule
                      
\end{tabular}

==> tables/incda_vs_uns.tex <==
\begin{tabular}{llcccccccc}
\toprule
 \textbf{Task}    & \textbf{Method}  &  \textbf{Metric}     &  {clear}     & partly cloudy & overcast & foggy & rainy           \\ \midrule
Semantic segmentation & Method~\cite{he2017mask} & mIoU (\%) $\uparrow$ &  34.2 & 34.8 & 36.7 & 8.70 &  19.9 & 13.4 & 4.34 \\
UDA & Method~\cite{he2017mask} & mIoU (\%) $\uparrow$ &  34.2 & - & - & - & 4.34 \\
IncrementalAdaptation & Method~\cite{he2017mask} & mIoU (\%) $\uparrow$ &  34.2 & 34.8 & 36.7 & 8.70 &  19.9 \\
\bottomrule
\end{tabular}

==> tables/mot_det.tex <==
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llccccc}
\toprule
\textbf{Dataset}                  & \multicolumn{1}{c}{\textbf{Training set}} & Task & AP  & MOTA           & MOTP           & IDF$_1$           \\ \midrule
\multirow{3}{*}{BDD100K} & MOT  & \multirow{3}{*}{Det}                             & 0.362   & 0.629          & 0.849          & 0.703          \\
                         & MOT + Det &                  &   \textbf{0.389}    & \textbf{0.639} & \textbf{0.850} & \textbf{0.713} \\ 
                         & Det  &                    & 0.370   & -          & -          & -          \\ \midrule
\multirow{3}{*}{Ours} & MOT &  \multirow{3}{*}{Det}                       &   0.454    & 0.659          & 0.880          & 0.760          \\
                         & MOT + Det &              &    \textbf{0.611}      & \textbf{0.674} & \textbf{0.885} & \textbf{0.774} \\
                         & Det &                    &   0.490    & -          & -         & -          \\
\bottomrule
\end{tabular}

==> tables/multitask.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3.3pt}
\center
\footnotesize
\begin{tabular}{lllcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Task}}                      & \multirow{2}{*}{\textbf{Train}} & \multirow{2}{*}{\textbf{Metric}}   & \multicolumn{1}{l}{\textbf{Source}} & \multicolumn{6}{c}{\textbf{OOD}}                                                                           & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{OOD avg.}}} & \multicolumn{1}{l}{\multirow{2}{*}{$\Delta$ \textbf{Source}}} & \multicolumn{1}{l}{\multirow{2}{*}{$\Delta$ \textbf{OOD}}} \\ \cmidrule(lr){4-4} \cmidrule{5-10} 
                                           &                        &                           & {clear}                      & {cloudy} & {overcast} & {foggy} & {rain} & {dawn/dusk} & {night} &                       &                        &                        \\ \midrule
\multirow{8}{*}{Semantic segmentation (S)}   & S                      & \multirow{8}{*}{mIoU (\%) $\uparrow$}     & 69.1                                & 40.6            & 40.6              & 21.5           & 19.6          & 18.1                 & 8.9                  & 24.9                                         & -                                             & -                                          \\
                                             & S + D                  &                                & \textbf{75.2}                       & {53.8}   & 52.6              & 24.3           & {26.6} & {24.0}        & {9.9}         & {31.9}                                & \textbf{8.9\%}                                & {28.1\%}                            \\
                                             & S + F                  &                                & 69.4                                & 51.8            & {54.7}     & {26.4}  & 22.4          & 22.7                 & 9.8                  & 31.3                                         & 0.4\%                                         & 25.8\%                                     \\
                                             & S + D + F              &                                & 71.8                                & 50.0            & 51.9              & 23.5           & 24.0          & 22.1                 & 9.5                  & 30.2                                         & 3.8\%                                         & 21.2\%                                     \\
                                             & S + I                  &                                & 74.8                                & \textbf{63.9}   & \textbf{68.1}     & \textbf{41.0}  & \textbf{36.8} & \textbf{37.3}        & \textbf{23.6}        & \textbf{45.1}                                & 8.2\%                                         & \textbf{81.3\%}                            \\
                                             & S + D + I              &                                & 75.0                                & 62.4            & 65.1              & 37.4           & 35.4          & 35.3                 & 20.5                 & 42.7                                         & 8.6\%                                         & 71.6\%                                     \\
                                             & S + F + I              &                                & 72.5                                & 58.3            & 59.6              & 35.8           & 27.2          & 28.8                 & 14.4                 & 37.3                                         & 4.9\%                                         & 50.1\%                                     \\
                                             & S + D + F + I          &                                & 74.7                                & 60.6            & 59.6              & 37.1           & 32.7          & 33.1               & 19.3           & 40.4                                         & 8.1\%                                         & 62.3\%                                      \\ \midrule
\multirow{8}{*}{Depth estimation (D)}        & D                      & \multirow{8}{*}{SILog $\downarrow$}         & 17.8                                & 28.3            & 23.1              & 81.9           & 46.3          & 54.6                 & 63.2                 & 49.6                                         & -                                             & -                                          \\
                                             & D + S                  &                                & 16.9                       & {25.2}   & 22.4              & {65.7}  & {43.0} & {49.4}        & 57.6                 & 43.9                                         & {5.6\%}                                & 13.0\%                                     \\
                                             & D + F                  &                                & 19.3                                & 25.3            & 20.4     & 66.6           & 45.3          & 50.3                 & {54.4}        & {43.7}                                & -7.8\%                                        & {13.4\%}                            \\
                                             & D + S + F              &                                & 19.6                                & 26.9            & 24.7              & 67.8           & 45.1          & 52.1                 & 56.6                 & 45.5                                         & -9.2\%                                        & 8.9\%                                      \\
                                             & D + I                  &                                & 17.3                                & 21.0            & 16.8              & 66.4           & 35.1          & 42.4                 & 48.4                 & 38.3                                         & 2.9\%                                         & 29.3\%                                     \\
                                             & D + S + I              &                                & \textbf{16.0}                       & \textbf{19.5}   & \textbf{15.4}     & 61.1           & \textbf{31.2} & \textbf{38.5}        & \textbf{42.7}        & \textbf{34.7}                                & \textbf{11.0\%}                               & \textbf{42.8\%}                            \\
                                             & D + F + I              &                                & 17.8                                & 21.4            & 17.9              & \textbf{47.9}  & 36.4          & 39.9                 & 46.3                 & 35.0                                         & 0.1\%                                         & 41.8\%                                     \\
                                             & D + S + F + I          &                                & 17.6                                & 21.9            & 18.3              & 53.2           & 37.1          & 42.7               & 50.5           & 37.3                                         & 1.0\%                                         & 33.0\%                                     \\ \midrule
\multirow{8}{*}{Optical flow estimation (F)} & F                      & \multirow{8}{*}{EPE (px) $\downarrow$}      & \textbf{6.0}                        & \textbf{6.7}    & \textbf{6.4}      & \textbf{9.0}   & \textbf{9.7}  & \textbf{9.1}         & \textbf{11.0}        & \textbf{8.6}                                 & \textbf{-}                                             & \textbf{-}                                          \\
                                             & F + S                  &                                & 7.8                                 & 8.3             & 8.5               & 10.4           & 12.0          & 10.9                 & 12.6                 & 10.4                                         & -23.1\%                                       & -17.4\%                                    \\
                                             & F + D                  &                                & {6.0}                        & 6.9             & {6.4}      & 9.4            & 10.4          & 9.6                  & 11.8                 & 9.1                                          & -0.2\%                                        & -5.0\%                                     \\
                                             & F + D + S              &                                & 6.1                                 & 8.5             & 8.3               & 10.6           & 12.1          & 11.0                 & 13.0                 & 10.6                                         & -2.1\%                                        & -18.5\%                                    \\
                                             & F + I                  &                                & 9.8                                 & 9.6             & 9.6               & 10.4           & 11.3          & 10.6                 & 12.1                 & 10.6                                         & -38.9\%                                       & -18.5\%                                    \\
                                             & F + S + I              &                                & 7.7                                 & 8.2             & 7.9               & 9.7            & 10.6          & 9.8                  & 11.8                 & 9.7                                          & -22.7\%                                       & -10.8\%                                    \\
                                             & F + D + I              &                                & 8.0                                 & 8.3             & 8.2               & 9.9            & 10.6          & 10.0                 & 11.9                 & 9.8                                          & -25.5\%                                       & -12.1\%                                    \\
                                             & F + D + S + I          &                                & 8.1                                 & 8.4             & 8.4               & 10.1           & 11.0          & 10.2               & 12.1           & 10.0                                         & -26.4\%                                       & -14.0\%                                    \\ \midrule
\multirow{8}{*}{Instance segmentation (I)}   & I                      & \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}mAP (\%) $\uparrow$ \\ (car)\end{tabular}} & 63.9                                & 57.4            & 65.7              & 21.9           & 31.2          & 22.7                 & 6.6                  & 34.2                                         & -                                             & -                                          \\
                                             & I + S                  &                                & 64.9                                & 59.1            & 66.2              & 26.4           & \textbf{34.4} & \textbf{27.1}                 & \textbf{14.3}                 & \textbf{37.9}                                         & 1.5\%                                         & \textbf{10.7\%}                            \\
                                             & I + S + D              &                                & 65.0                                & 57.9            & 64.9              & 25.9           & 32.6          & 26.1                 & 10.9                 & 36.4                                         & 1.6\%                                         & 6.3\%                                      \\
                                             & I + S + F              &                                & 62.3                                & 57.1            & 64.2              & 21.6           & 31.6          & 23.6                 & 7.7                  & 34.3                                         & -2.5\%                                        & 0.1\%                                      \\
                                             & I + D                  &                                & \textbf{65.9}                       & \textbf{59.3}   & 66.9              & \textbf{26.8}  & 32.2          & 26.3                 & 11.4                 & 37.2                                         & \textbf{3.1\%}                                & 8.5\%                                      \\
                                             & I + D + F              &                                & 65.8                                & 50.2            & \textbf{67.0}     & 21.5           & 31.0          & 22.9                 & 6.7                  & 33.2                                         & 2.9\%                                         & -3.0\%                                     \\
                                             & I + F                  &                                & 63.1                                & 56.9            & 65.1              & 20.4           & 28.9          & 21.7                 & 5.0                  & 33.0                                         & -1.3\%                                        & -3.6\%                                     \\
                                             & I + S + D + F          &                                & 64.8                                & 57.9            & 65.3              & 22.8           & 31.5          & 23.1               & 8.3            & 34.8                                         & 1.4\%                                         & 1.6\%                               \\ \bottomrule
\end{tabular}
\caption{Multitask learning performances. We evaluate 15 combinations of 4 perception tasks: semantic segmentation (S), monocular depth estimation (D), optical flow estimation (F), and instance segmentation (I). The combinations of S + I, S + D, and S + D + I significantly improve on both tasks' source and OOD performance in their respective tasks. $\uparrow$ ($\downarrow$): the higher (lower) the better.}
\label{tab:multitask_four_tasks}
\end{table*}

==> tables/multitask_shift.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Training Tasks   & Target Task         & Metric                & Daytime & Dawn/Dusk & Night &  \\ \hline
OF               & \multirow{8}{*}{OF} & \multirow{8}{*}{EPE}  &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + D           &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + SS          &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + IS          &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + D + SS      &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + D + IS      &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + IS + SS     &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
OF + IS + SS + D &                     &                       &         &           &       &  \\ \hline
                 &                     &                       &         &           &       &  \\ \hline
                 &                     &                       &         &           &       &  \\ \hline
                 &                     &                       &         &           &       &  \\ \hline
D                & \multirow{8}{*}{D}  & \multirow{8}{*}{RMSE} &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + OF           &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + SS           &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + IS           &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + SS + OF      &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + OF + IS      &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + IS + SS      &                     &                       &         &           &       &  \\ \cline{1-1} \cline{4-7} 
D + IS + SS + OF &                     &                       &         &           &       &  \\ \hline
IS               & IS                  & AP                    &         &           &       &  \\ \hline
....             &                     &                       &         &           &       &  \\ \hline
SS               & SS                  & AP                    &         &           &       &  \\ \hline
...              &                     &                       &         &           &       &  \\ \hline
\end{tabular}
\end{table}

==> tables/seg_det.tex <==
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llcccc}
\toprule
\textbf{Dataset}                  & \multicolumn{1}{c}{\textbf{Training set}} & Task & AP            & AP$_{50}$     & AP$_{75}$     \\ \midrule
\multirow{4}{*}{BDD100K} & InsSeg & \multirow{2}{*}{InsSeg}                           & 0.218          & 0.405          & 0.205          \\
                         & InsSeg + Det &                                             & \textbf{0.245} & \textbf{0.454} & \textbf{0.216} \\ \cline{3-6} 
                         & InsSeg + Det &  \multirow{2}{*}{Det}                     & ... & ... & ... \\ 
                         & Det &                                                    & ... & ... & ... \\ \midrule
\multirow{4}{*}{Ours} & InsSeg & \multirow{2}{*}{InsSeg}                            &                            0.342          & 0.610          & 0.349          \\
                         & InsSeg + Det &                                             & \textbf{0.363} & \textbf{0.668} & \textbf{0.355} \\ \cline{3-6}
                         & InsSeg + Det &  \multirow{2}{*}{Det}                     & ... & ... & ... \\
                         & Det &                                                    & ... & ... & ... \\ 
% \multirow{2}{*}{Ours}    & InsSeg                           & 0.342          & 0.610          & 0.349          \\
%                          & InsSeg + Det                     & \textbf{0.363} & \textbf{0.668} & \textbf{0.355} \\
\bottomrule
\end{tabular}

==> tables/sem_seg.tex <==
\begin{tabular}{@{}llcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{In-domain}} & \multicolumn{2}{c}{\textbf{OOD avg.}} \\ \cmidrule(r){3-4} \cmidrule(c){5-6}
                         & \multicolumn{1}{c}{} & Acc            & mIoU           & Acc            & mIoU           \\
                         \midrule
\multirow{3}{*}{{BDD100K}} & FCN                  & 90.44          & 44.86          & 52.58          & 25.49          \\
                         & DRN-D                & 91.28          & 49.04          & 53.07          & 27.86          \\
                         & DeepLab v3+          & \textbf{91.96} & \textbf{51.21} & \textbf{53.47} & \textbf{29.10} \\ \midrule
\multirow{3}{*}{{Ours}}    & FCN                  & 98.05          & 77.46          & 58.02          & 44.01          \\
                         & DRN-D                & 98.56          & 83.61          & 58.32          & 47.51          \\
                         & DeepLab v3+          & \textbf{98.77} & \textbf{83.85} & \textbf{58.44} & \textbf{47.64} \\
\bottomrule
\end{tabular}


==> tables/unc.tex <==
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llcccccccc}
% \toprule
 & \textbf{Method}  &
  \parbox[t]{5mm}{\rotatebox[origin=l]{90}{\shortstack[l]{clear-\\daytime}}} &
  \parbox[t]{2mm}{\rotatebox[origin=l]{90}{cloudy}} &
  \parbox[t]{2mm}{\rotatebox[origin=l]{90}{overcast}} &
  \parbox[t]{2mm}{\rotatebox[origin=l]{90}{foggy}} &
  \parbox[t]{2mm}{\rotatebox[origin=l]{90}{rainy}} &
  \parbox[t]{2mm}{\rotatebox[origin=l]{90}{dawn/\\dusk}} &
  \parbox[t]{2mm}{\rotatebox[origin=l]{90}{night}} & 
  \parbox[t]{5mm}{\rotatebox[origin=l]{90}{\textbf{\shortstack[l]{OOD\\avg.}}}} \\ \midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{SHIFT}}}}  & Softmax  & 86.9 & 83.8 & 73.5 & 63.3 & 28.4 & 65.6 & 7.1 & 53.6 \\
& MCDO & 93.4 & 71.7 & 73.4 & 62.3 & 74.2 & 31.2 & 48.4 & 61.1 \\
    & Ensemble & 94.9 & 83.5 & 83.5 & 71.3 & 78.4 & 65.6 & 43.1 & 70.9 \\\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{BDD}}}} & Softmax & 69.4 & 58.2 & 81.8 & 84.1 & 83.5 & 77.9 & 47.0 & 72.1 \\
& MCDO & 74.2 & 55.5 & 81.2 & 83.8 & 77.4 & 78.1 & 50.0 & 69.6 \\
& Ensemble & 82.6 & 58.8 & 79.2 & 81.7 & 81.8 & 80.9 & 58.5 & 73.5 \\
                      \bottomrule
\end{tabular}

% \begin{tabular}{llccc}
% \toprule
%                   & \multicolumn{1}{l}{\textbf{Domain}} & \multicolumn{1}{l}{Softmax} & \multicolumn{1}{l}{MCD~\cite{gal2016dropout}} & \multicolumn{1}{l}{ Ensemble~\cite{lakshminarayanan2017simple}} \\ \midrule
% \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{SHIFT}}}} & \underline{clear-daytime}           & 86.9                        & 93.4                                                 & 94.9                                                                 \\
%                   & partly cloudy                       & 83.8                        & 71.7                                                 & 83.5                                                                 \\
%                   & overcast                            & 73.5                        & 73.4                                                 & 83.5                                                                 \\
%                   & foggy                               & 63.3                        & 62.29                                                & 71.3                                                                 \\
%                   & rainy                               & 28.4                        & 74.2                                                 & 78.4                                                                 \\
%                   & dawn/dusk                           & 65.6                        & 31.2                                                 & 65.6                                                                 \\
%                   & night                               & 7.1                         & 48.4                                                 & 43.1                                                                 \\
%                   & \textbf{OOD Avg.}                    & 53.6                        & 61.1                                                 & 70.9                                                                 \\ \midrule
% \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{BDD100K}}}} & \underline{clear-daytime}           & 69.4                        & 74.2                                                 & 82.6                                                                 \\
%                   & partly cloudy                       & 58.2                        & 55.5                                                 & 58.8                                                                 \\
%                   & overcast                            & 81.8                        & 81.2                                                 & 79.2                                                                 \\
%                   & foggy                               & 84.1                        & 83.8                                                 & 81.7                                                                 \\
%                   & rainy                               & 83.5                        & 77.4                                                 & 81.8                                                                 \\
%                   & dawn/dusk                           & 77.9                        & 78.1                                                 & 80.9                                                                 \\
%                   & night                               & 47.0                        & 50.0                                                 & 58.5                                                                 \\ 
%                   & \textbf{OOD Avg.}                    & 72.1                        & 69.6                                                 & 73.5                                                                 \\ \bottomrule
% \end{tabular}
